Hybrid mimetic finite-difference and virtual element formulation for coupled poromechanics

We present a hybrid mimetic finite-difference and virtual element formulation for coupled single-phase poromechanics on unstructured meshes. The key advantage of the scheme is that it is convergent on complex meshes containing highly distorted cells with arbitrary shapes. We use a local pressure-jump stabilization method based on unstructured macro-elements to prevent the development of spurious pressure modes in incompressible problems approaching undrained conditions. A scalable linear solution strategy is obtained using a block-triangular preconditioner designed specifically for the saddle-point systems arising from the proposed discretization. The accuracy and efficiency of our approach are demonstrated numerically on two-dimensional benchmark problems.

==> plotData/convergenceTest/Meshes/Cartesian.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=.75\linewidth,
height=.75\linewidth,
xmin=-0.1,
xmax=1.1,
ymin=-0.1,
ymax=1.1,
axis line style={draw=black},
xtick={0.0,1.0},
ytick={0.0,1.0},
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]

\addplot[area legend, table/row sep=crcr, patch, patch type=rectangle, fill=white, faceted color=black, patch table={%
6	8	9	7\\
7	9	13	12\\
12	13	11	10\\
8	2	4	9\\
9	4	5	13\\
13	5	3	11\\
2	1	14	4\\
4	14	15	5\\
5	15	0	3\\
}]
table[row sep=crcr] {%
x	y\\
1.00000000083746	1.00000000083746\\
1.00000000083746	8.77259653808693e-11\\
0.666666666666667	8.77259931364449e-11\\
0.666666666666667	1.00000000083746\\
0.666666666666667	0.333333333333333\\
0.666666666666667	0.666666666666667\\
8.77259653808693e-11	8.77259653808693e-11\\
8.77259653808693e-11	0.333333333333333\\
0.333333333333333	8.77259653808693e-11\\
0.333333333333333	0.333333333333333\\
8.77259653808693e-11	1.00000000083746\\
0.333333333333333	1.00000000083746\\
8.77259376252937e-11	0.666666666666667\\
0.333333333333333	0.666666666666667\\
1.00000000083746	0.333333333333333\\
1.00000000083746	0.666666666666667\\
};
%\addlegendentry{data1}

\end{axis}

\end{tikzpicture}%

==> plotData/convergenceTest/Meshes/Polymesher1.tex <==
\begin{tikzpicture}
  \begin{axis}[%
    width=.75\linewidth, height=.75\linewidth, xmin=-0.1, xmax=1.1,
    ymin=-0.1, ymax=1.1, axis line style={draw=black},
    xtick={0.0,1.0}, ytick={0.0,1.0}, axis x line*=bottom, axis y
    line*=left, legend style={legend cell align=left, align=left,
      draw=white!15!black} ]

    \addplot[area legend, table/row sep=crcr, patch, patch
    type=polygon, vertex count=8, fill=white, faceted color=black,
    patch table={%
      15	26	24	10	12	11	13	14\\
      19	20	21	16	18	17	23	22\\
      4	15	14	3	3 3 3 3\\
      10	9	8	6	12	12 12 12\\
      22	23	24	26	25	25 25 25\\
      0	2	7	25	26	15	4	1\\
      5	20	19	7	2	2 2 2\\
      19	22	25	7	7 7 7 7\\
      23	17	9	10	24	24 24 24\\
    }] table[row sep=crcr] {%
      x	y\\
      9.2373664273282e-11	0.409669627145423\\
      9.23736920288576e-11	0.882678167005679\\
      1.29307592411365e-10	0.409669627113969\\
      1.36151812046847e-10	1.00000000035112\\
      1.36151812046847e-10	0.882678167083799\\
      1.29307592411365e-10	1.01207459080044e-10\\
      1.0000000004729	1.00000000024913\\
      0.222931695738912	0.441301022064936\\
      1.0000000004729	0.865984921655418\\
      1.00000000036485	0.865984921559573\\
      0.812504435668387	0.844533945631048\\
      0.763575589788501	1.00000000061377\\
      0.763575590060077	1.00000000024913\\
      0.479035640844754	1.00000000061377\\
      0.479035640723704	1.00000000035112\\
      0.445223088753573	0.73048080090985\\
      1.00000000082303	9.80451275722771e-11\\
      1.00000000036485	0.455668806598631\\
      1.00000000082303	0.455668806410652\\
      0.540076582455247	0.104809950926165\\
      0.53901028111446	1.01207403568893e-10\\
      0.539010281116488	9.80451275722771e-11\\
      0.684002978313814	0.346906158026769\\
      0.985327450283223	0.45799069980968\\
      0.759017237504133	0.727672098906249\\
      0.446115291206573	0.673742852259708\\
      0.453899254195495	0.707780708838692\\
    };

  \end{axis}
\end{tikzpicture}%

==> plotData/convergenceTest/Meshes/Polymesher20.tex <==
% This file was created by matlab2tikz.
%
% The latest updates can be retrieved from
% http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
% where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

  \begin{axis}[%
    width=.75\linewidth,
    height=.75\linewidth,
    xmin=-0.1,
    xmax=1.1,
    ymin=-0.1,
    ymax=1.1,
    axis line style={draw=black},
    xtick={0.0,1.0},
    ytick={0.0,1.0},
    axis x line*=bottom,
    axis y line*=left,
    legend style={legend cell align=left, align=left, draw=white!15!black}
    ]

    \addplot[area legend, table/row sep=crcr, patch, patch type=polygon, vertex count=7, fill=white, faceted color=black, patch table={%
      0	14	12	5	7	7 7\\
      3	1	2	24	25	10	11\\
      26	9	0	7	8	27	27\\
      12	13	22	23	4	6	5\\
      15	11	10	13	12	14	14\\
      17	16	15	14	0	9	9\\
      19	20	21	16	17	18	18\\
      21	3	11	15	16	16 16\\
      10	25	22	13	13 13 13\\
    }]
    table[row sep=crcr] {%
      x	y\\
      0.32123220030744	0.680650268076965\\
      0.647434517763152	8.6062046378288e-11\\
      1.00000000088766	8.60620186227123e-11\\
      0.647434517758247	9.10546360533004e-11\\
      1.00000000087098	1.00000000083656\\
      0.655502792477606	1.00000000083393\\
      0.655502792480159	1.00000000083656\\
      0.320456424538895	1.00000000083393\\
      0.320456424534834	1.00000000083791\\
      9.85876935644114e-11	0.652150736677953\\
      0.694210351300406	0.3437959391264\\
      0.656096083362804	0.312757164904515\\
      0.655038715275374	0.696277258788796\\
      0.705069488086812	0.652967148646889\\
      0.363578445210751	0.642868099584632\\
      0.36750723480647	0.367194481385205\\
      0.316332137677288	0.321491714283174\\
      9.85876658088358e-11	0.350575468463656\\
      8.24323664883053e-11	0.350575468447013\\
      8.24323387327297e-11	8.83483564084742e-11\\
      0.321430136100528	8.83483564084742e-11\\
      0.321430136103373	9.10546638088761e-11\\
      1.00000000072519	0.678306857311166\\
      1.00000000087098	0.678306857448304\\
      1.00000000088766	0.314040529546172\\
      1.00000000072519	0.314040529703114\\
      8.31044122406865e-11	0.652150736694072\\
      8.31043844851109e-11	1.00000000083791\\
    };

  \end{axis}
\end{tikzpicture}%

==> plotData/convergenceTest/Meshes/Skewed.tex <==
\begin{tikzpicture}

  \begin{axis}[%
    width=.75\linewidth,
    height=.75\linewidth,
    xmin=-0.1,
    xmax=1.1,
    ymin=-0.1,
    ymax=1.1,
    axis line style={draw=black},
    xtick={0.0,1.0},
    ytick={0.0,1.0},
    axis x line*=bottom,
    axis y line*=left,
    legend style={legend cell align=left, align=left, draw=white!15!black}
    ]

    \addplot[area legend, table/row sep=crcr, patch, patch type=rectangle, fill=white, faceted color=black, patch table={%
      6	8	9	7\\
      7	9	13	12\\
      12	13	11	10\\
      8	2	4	9\\
      9	4	5	13\\
      13	5	3	11\\
      2	1	14	4\\
      4	14	15	5\\
      5	15	0	3\\
    }]
    table[row sep=crcr] {%
      x	y\\
      1.00000000083746	1.00000000083746\\
      1.00000000083746	8.77259645687686e-11\\
      0.666666666599837	2.08967131034658e-11\\
      0.666666666028693	1.00000000019949\\
      0.719166666666667	0.385833333333333\\
      0.614166666666667	0.614166666666667\\
      8.77259652957998e-11	8.77259652957998e-11\\
      1.54555231479424e-10	0.333333333400163\\
      0.333333333400163	1.5455523195311e-10\\
      0.280833333333333	0.280833333333333\\
      8.77259645687686e-11	1.00000000083746\\
      0.333333333971307	1.00000000147543\\
      2.08966926708181e-11	0.666666666599837\\
      0.385833333333333	0.719166666666667\\
      1.00000000147543	0.333333333971307\\
      1.00000000019949	0.666666666028693\\
    };
    % \addlegendentry{data1}

  \end{axis}
\end{tikzpicture}%

==> plotData/mandelTest/Cartesian/solution_fullycoupled_01000.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=1,
xlabel style={font=\color{white!15!black}},
xlabel={x},
ymin=0,
ymax=1.2,
axis background/.style={fill=white},
title style={font=\bfseries},
title={Pressure profile, t = 9.000000e+01},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, draw=none, mark=o, mark options={solid, mycolor1}]
  table[]{plotData/mandelTest/Cartesian/solution_fullycoupled_01000-1.tsv};
\addlegendentry{data1}

\addplot [color=mycolor2]
  table[]{plotData/mandelTest/Cartesian/solution_fullycoupled_01000-2.tsv};
\addlegendentry{data2}

\end{axis}
\end{tikzpicture}%

==> plotData/mandelTest/Cartesian/solution_fullycoupled_03000.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=1,
xlabel style={font=\color{white!15!black}},
xlabel={x},
ymin=0,
ymax=0.9,
axis background/.style={fill=white},
title style={font=\bfseries},
title={Pressure profile, t = 2.700000e+02},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, draw=none, mark=o, mark options={solid, mycolor1}]
  table[]{plotData/mandelTest/Cartesian/solution_fullycoupled_03000-1.tsv};
\addlegendentry{data1}

\addplot [color=mycolor2]
  table[]{plotData/mandelTest/Cartesian/solution_fullycoupled_03000-2.tsv};
\addlegendentry{data2}

\end{axis}
\end{tikzpicture}%

==> plotData/mandelTest/Cartesian/solution_fullycoupled_06000.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=1,
xlabel style={font=\color{white!15!black}},
xlabel={x},
ymin=0,
ymax=0.6,
axis background/.style={fill=white},
title style={font=\bfseries},
title={Pressure profile, t = 5.400000e+02},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, draw=none, mark=o, mark options={solid, mycolor1}]
  table[]{plotData/mandelTest/Cartesian/solution_fullycoupled_06000-1.tsv};
\addlegendentry{data1}

\addplot [color=mycolor2]
  table[]{plotData/mandelTest/Cartesian/solution_fullycoupled_06000-2.tsv};
\addlegendentry{data2}

\end{axis}
\end{tikzpicture}%

==> plotData/mandelTest/Cartesian/solution_fullycoupled_10000.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=1,
xlabel style={font=\color{white!15!black}},
xlabel={x},
ymin=0,
ymax=0.3,
axis background/.style={fill=white},
title style={font=\bfseries},
title={Pressure profile, t = 9.000000e+02},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, draw=none, mark=o, mark options={solid, mycolor1}]
  table[]{plotData/mandelTest/Cartesian/solution_fullycoupled_10000-1.tsv};
\addlegendentry{data1}

\addplot [color=mycolor2]
  table[]{plotData/mandelTest/Cartesian/solution_fullycoupled_10000-2.tsv};
\addlegendentry{data2}

\end{axis}
\end{tikzpicture}%

==> plotData/mandelTest/Hybrid/solution_fullycoupled_01000.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=1,
xlabel style={font=\color{white!15!black}},
xlabel={x},
ymin=0,
ymax=1.2,
axis background/.style={fill=white},
title style={font=\bfseries},
title={Pressure profile, t = 9.000000e+01},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, draw=none, mark=o, mark options={solid, mycolor1}]
  table[]{plotData/mandelTest/Hybrid/solution_fullycoupled_01000-1.tsv};
\addlegendentry{data1}

\addplot [color=mycolor2]
  table[]{plotData/mandelTest/Hybrid/solution_fullycoupled_01000-2.tsv};
\addlegendentry{data2}

\end{axis}
\end{tikzpicture}%

==> plotData/mandelTest/Hybrid/solution_fullycoupled_03000.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=1,
xlabel style={font=\color{white!15!black}},
xlabel={x},
ymin=0,
ymax=0.9,
axis background/.style={fill=white},
title style={font=\bfseries},
title={Pressure profile, t = 2.700000e+02},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, draw=none, mark=o, mark options={solid, mycolor1}]
  table[]{plotData/mandelTest/Hybrid/solution_fullycoupled_03000-1.tsv};
\addlegendentry{data1}

\addplot [color=mycolor2]
  table[]{plotData/mandelTest/Hybrid/solution_fullycoupled_03000-2.tsv};
\addlegendentry{data2}

\end{axis}
\end{tikzpicture}%

==> plotData/mandelTest/Hybrid/solution_fullycoupled_06000.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=1,
xlabel style={font=\color{white!15!black}},
xlabel={x},
ymin=0,
ymax=0.6,
axis background/.style={fill=white},
title style={font=\bfseries},
title={Pressure profile, t = 5.400000e+02},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, draw=none, mark=o, mark options={solid, mycolor1}]
  table[]{plotData/mandelTest/Hybrid/solution_fullycoupled_06000-1.tsv};
\addlegendentry{data1}

\addplot [color=mycolor2]
  table[]{plotData/mandelTest/Hybrid/solution_fullycoupled_06000-2.tsv};
\addlegendentry{data2}

\end{axis}
\end{tikzpicture}%

==> plotData/mandelTest/Hybrid/solution_fullycoupled_10000.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=1,
xlabel style={font=\color{white!15!black}},
xlabel={x},
ymin=0,
ymax=0.3,
axis background/.style={fill=white},
title style={font=\bfseries},
title={Pressure profile, t = 9.000000e+02},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, draw=none, mark=o, mark options={solid, mycolor1}]
  table[]{plotData/mandelTest/Hybrid/solution_fullycoupled_10000-1.tsv};
\addlegendentry{data1}

\addplot [color=mycolor2]
  table[]{plotData/mandelTest/Hybrid/solution_fullycoupled_10000-2.tsv};
\addlegendentry{data2}

\end{axis}
\end{tikzpicture}%

==> plotData/mandelTest/Polymesher1/solution_fullycoupled_01000.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=1,
xlabel style={font=\color{white!15!black}},
xlabel={x},
ymin=0,
ymax=1.2,
axis background/.style={fill=white},
title style={font=\bfseries},
title={Pressure profile, t = 9.000000e+01},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, draw=none, mark=o, mark options={solid, mycolor1}]
  table[]{plotData/mandelTest/Polymesher1/solution_fullycoupled_01000-1.tsv};
\addlegendentry{data1}

\addplot [color=mycolor2]
  table[]{plotData/mandelTest/Polymesher1/solution_fullycoupled_01000-2.tsv};
\addlegendentry{data2}

\end{axis}
\end{tikzpicture}%

==> plotData/mandelTest/Polymesher1/solution_fullycoupled_03000.tex <==
\begin{tikzpicture}

  \begin{axis}[%
    width=\textwidth,
    height=\textwidth,
    xmin=0,
    xmax=1,
    xlabel style={font=\color{white!15!black}},
    xlabel={$x$},
    ymin=0,
    ymax=0.90,
    axis background/.style={fill=white},
    legend style={font=\small},
    tick label style={font=\small},
    label style={font=\small},
    ]
    \addplot [color=mycolor1, draw=none, mark=o, mark options={solid, mycolor1}]
    table[]{plotData/mandelTest/Polymesher20/solution_fullycoupled_03000-1.tsv};
    \addlegendentry{Computed values.}

    \addplot [color=mycolor2]
    table[]{plotData/mandelTest/Polymesher20/solution_fullycoupled_03000-2.tsv};
    \addlegendentry{Exact solution.}

  \end{axis}
\end{tikzpicture}%

==> plotData/mandelTest/Polymesher1/solution_fullycoupled_06000.tex <==
\begin{tikzpicture}

  \begin{axis}[%
    width=\textwidth,
    height=\textwidth,
    xmin=0,
    xmax=1,
    xlabel style={font=\color{white!15!black}},
    xlabel={$x$},
    ymin=0,
    ymax=0.90,
    axis background/.style={fill=white},
    legend style={font=\small},
    tick label style={font=\small},
    label style={font=\small},
    ]
    \addplot [color=mycolor1, draw=none, mark=o, mark options={solid, mycolor1}]
    table[]{plotData/mandelTest/Polymesher20/solution_fullycoupled_06000-1.tsv};
    \addlegendentry{Computed values.}

    \addplot [color=mycolor2]
    table[]{plotData/mandelTest/Polymesher20/solution_fullycoupled_06000-2.tsv};
    \addlegendentry{Exact solution.}

  \end{axis}
\end{tikzpicture}%

==> plotData/mandelTest/Polymesher1/solution_fullycoupled_10000.tex <==
\begin{tikzpicture}
  \begin{axis}[%
    width=\textwidth,
    height=\textwidth,
    xmin=0,
    xmax=1,
    xlabel style={font=\color{white!15!black}},
    xlabel={$x$},
    ymin=0,
    ymax=0.90,
    axis background/.style={fill=white},
    legend style={font=\small},
    tick label style={font=\small},
    label style={font=\small},
    ]
    \addplot [color=mycolor1, draw=none, mark=o, mark options={solid, mycolor1}]
    table[]{plotData/mandelTest/Polymesher20/solution_fullycoupled_10000-1.tsv};
    \addlegendentry{Computed values.}

    \addplot [color=mycolor2]
    table[]{plotData/mandelTest/Polymesher20/solution_fullycoupled_10000-2.tsv};
    \addlegendentry{Exact solution.}

  \end{axis}
\end{tikzpicture}%

==> plotData/mandelTest/Polymesher20/solution_fullycoupled_01000.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=1,
xlabel style={font=\color{white!15!black}},
xlabel={x},
ymin=0,
ymax=1.2,
axis background/.style={fill=white},
title style={font=\bfseries},
title={Pressure profile, t = 9.000000e+01},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, draw=none, mark=o, mark options={solid, mycolor1}]
  table[]{plotData/mandelTest/Polymesher20/solution_fullycoupled_01000-1.tsv};
\addlegendentry{data1}

\addplot [color=mycolor2]
  table[]{plotData/mandelTest/Polymesher20/solution_fullycoupled_01000-2.tsv};
\addlegendentry{data2}

\end{axis}
\end{tikzpicture}%

==> plotData/mandelTest/Polymesher20/solution_fullycoupled_03000.tex <==
\begin{tikzpicture}

  \begin{axis}[%
    width=\textwidth,
    height=\textwidth,
    xmin=0,
    xmax=1,
    xlabel style={font=\color{white!15!black}},
    xlabel={$x$},
    ymin=0,
    ymax=0.90,
    axis background/.style={fill=white},
    legend style={font=\small},
    tick label style={font=\small},
    label style={font=\small},
    ]
    \addplot [color=mycolor1, draw=none, mark=o, mark options={solid, mycolor1}]
    table[]{plotData/mandelTest/Polymesher20/solution_fullycoupled_03000-1.tsv};
    \addlegendentry{Computed values.}

    \addplot [color=mycolor2]
    table[]{plotData/mandelTest/Polymesher20/solution_fullycoupled_03000-2.tsv};
    \addlegendentry{Exact solution.}

  \end{axis}
\end{tikzpicture}%

==> plotData/mandelTest/Polymesher20/solution_fullycoupled_06000.tex <==
\begin{tikzpicture}

  \begin{axis}[%
    width=\textwidth,
    height=\textwidth,
    xmin=0,
    xmax=1,
    xlabel style={font=\color{white!15!black}},
    xlabel={$x$},
    ymin=0,
    ymax=0.90,
    axis background/.style={fill=white},
    legend style={font=\small},
    tick label style={font=\small},
    label style={font=\small},
    ]
    \addplot [color=mycolor1, draw=none, mark=o, mark options={solid, mycolor1}]
    table[]{plotData/mandelTest/Polymesher20/solution_fullycoupled_06000-1.tsv};
    \addlegendentry{Computed values.}

    \addplot [color=mycolor2]
    table[]{plotData/mandelTest/Polymesher20/solution_fullycoupled_06000-2.tsv};
    \addlegendentry{Exact solution.}

  \end{axis}
\end{tikzpicture}%

==> plotData/mandelTest/Polymesher20/solution_fullycoupled_10000.tex <==
\begin{tikzpicture}
  \begin{axis}[%
    width=\textwidth,
    height=\textwidth,
    xmin=0,
    xmax=1,
    xlabel style={font=\color{white!15!black}},
    xlabel={$x$},
    ymin=0,
    ymax=0.90,
    axis background/.style={fill=white},
    legend style={font=\small},
    tick label style={font=\small},
    label style={font=\small},
    ]
    \addplot [color=mycolor1, draw=none, mark=o, mark options={solid, mycolor1}]
    table[]{plotData/mandelTest/Polymesher20/solution_fullycoupled_10000-1.tsv};
    \addlegendentry{Computed values.}

    \addplot [color=mycolor2]
    table[]{plotData/mandelTest/Polymesher20/solution_fullycoupled_10000-2.tsv};
    \addlegendentry{Exact solution.}

  \end{axis}
\end{tikzpicture}%

==> plotData/mandelTest/Skewed/solution_fullycoupled_01000.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=1,
xlabel style={font=\color{white!15!black}},
xlabel={x},
ymin=0,
ymax=1.2,
axis background/.style={fill=white},
title style={font=\bfseries},
title={Pressure profile, t = 9.000000e+01},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, draw=none, mark=o, mark options={solid, mycolor1}]
  table[]{plotData/mandelTest/Skewed/solution_fullycoupled_01000-1.tsv};
\addlegendentry{data1}

\addplot [color=mycolor2]
  table[]{plotData/mandelTest/Skewed/solution_fullycoupled_01000-2.tsv};
\addlegendentry{data2}

\end{axis}
\end{tikzpicture}%

==> plotData/mandelTest/Skewed/solution_fullycoupled_03000.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=1,
xlabel style={font=\color{white!15!black}},
xlabel={x},
ymin=0,
ymax=0.9,
axis background/.style={fill=white},
title style={font=\bfseries},
title={Pressure profile, t = 2.700000e+02},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, draw=none, mark=o, mark options={solid, mycolor1}]
  table[]{plotData/mandelTest/Skewed/solution_fullycoupled_03000-1.tsv};
\addlegendentry{data1}

\addplot [color=mycolor2]
  table[]{plotData/mandelTest/Skewed/solution_fullycoupled_03000-2.tsv};
\addlegendentry{data2}

\end{axis}
\end{tikzpicture}%

==> plotData/mandelTest/Skewed/solution_fullycoupled_06000.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=1,
xlabel style={font=\color{white!15!black}},
xlabel={x},
ymin=0,
ymax=0.6,
axis background/.style={fill=white},
title style={font=\bfseries},
title={Pressure profile, t = 5.400000e+02},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, draw=none, mark=o, mark options={solid, mycolor1}]
  table[]{plotData/mandelTest/Skewed/solution_fullycoupled_06000-1.tsv};
\addlegendentry{data1}

\addplot [color=mycolor2]
  table[]{plotData/mandelTest/Skewed/solution_fullycoupled_06000-2.tsv};
\addlegendentry{data2}

\end{axis}
\end{tikzpicture}%

==> plotData/mandelTest/Skewed/solution_fullycoupled_10000.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=1,
xlabel style={font=\color{white!15!black}},
xlabel={x},
ymin=0,
ymax=0.3,
axis background/.style={fill=white},
title style={font=\bfseries},
title={Pressure profile, t = 9.000000e+02},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, draw=none, mark=o, mark options={solid, mycolor1}]
  table[]{plotData/mandelTest/Skewed/solution_fullycoupled_10000-1.tsv};
\addlegendentry{data1}

\addplot [color=mycolor2]
  table[]{plotData/mandelTest/Skewed/solution_fullycoupled_10000-2.tsv};
\addlegendentry{data2}

\end{axis}
\end{tikzpicture}%

==> plotData/mandelTest/solution_fullycoupled_01000.tex <==
\begin{tikzpicture}

  \begin{axis}[%
    width=\textwidth,
    height=\textwidth,
    xmin=0,
    xmax=1,
    xlabel style={font=\color{white!15!black}},
    xlabel={$x$},
    ymin=0,
    ymax=1.2,
    axis background/.style={fill=white},
    legend style={font=\small},
    tick label style={font=\small},
    label style={font=\small},
    ]
    \addplot [color=mycolor2, draw=none, mark=o, mark options={solid, mycolor2}]
    table[]{plotData/mandelTest/Polymesher20/solution_fullycoupled_01000-1.tsv};
    \addlegendentry{\texttt{Polymesher20}.}

    \addplot [color=mycolor3, draw=none, mark=square, mark options={solid, mycolor3}]
    table[]{plotData/mandelTest/Polymesher1/solution_fullycoupled_01000-1.tsv};
    \addlegendentry{\texttt{Polymesher1}.}


    \addplot [color=mycolor1]
    table[]{plotData/mandelTest/Polymesher20/solution_fullycoupled_01000-2.tsv};
    \addlegendentry{Exact solution.}

  \end{axis}
\end{tikzpicture}%

==> plotData/mandelTest/solution_fullycoupled_03000.tex <==
\begin{tikzpicture}

  \begin{axis}[%
    width=\textwidth,
    height=\textwidth,
    xmin=0,
    xmax=1,
    xlabel style={font=\color{white!15!black}},
    xlabel={$x$},
    ymin=0,
    ymax=0.90,
    axis background/.style={fill=white},
    legend style={font=\small},
    tick label style={font=\small},
    label style={font=\small},
    ]
    \addplot [color=mycolor2, draw=none, mark=o, mark options={solid, mycolor2}]
    table[]{plotData/mandelTest/Polymesher20/solution_fullycoupled_03000-1.tsv};
    \addlegendentry{\texttt{Polymesher20}.}

    \addplot [color=mycolor3, draw=none, mark=square, mark options={solid, mycolor3}]
    table[]{plotData/mandelTest/Polymesher1/solution_fullycoupled_03000-1.tsv};
    \addlegendentry{\texttt{Polymesher1}.}


    \addplot [color=mycolor1]
    table[]{plotData/mandelTest/Polymesher20/solution_fullycoupled_03000-2.tsv};
    \addlegendentry{Exact solution.}

  \end{axis}
\end{tikzpicture}%

==> plotData/mandelTest/solution_fullycoupled_06000.tex <==
\begin{tikzpicture}

  \begin{axis}[%
    width=\textwidth,
    height=\textwidth,
    xmin=0,
    xmax=1,
    xlabel style={font=\color{white!15!black}},
    xlabel={$x$},
    ymin=0,
    ymax=0.90,
    axis background/.style={fill=white},
    legend style={font=\small},
    tick label style={font=\small},
    label style={font=\small},
    ]
    \addplot [color=mycolor2, draw=none, mark=o, mark options={solid, mycolor2}]
    table[]{plotData/mandelTest/Polymesher20/solution_fullycoupled_06000-1.tsv};
    \addlegendentry{\texttt{Polymesher20}.}

    \addplot [color=mycolor3, draw=none, mark=square, mark options={solid, mycolor3}]
    table[]{plotData/mandelTest/Polymesher1/solution_fullycoupled_06000-1.tsv};
    \addlegendentry{\texttt{Polymesher1}.}

    \addplot [color=mycolor1]
    table[]{plotData/mandelTest/Polymesher20/solution_fullycoupled_06000-2.tsv};
    \addlegendentry{Exact solution.}

  \end{axis}
\end{tikzpicture}%

==> plotData/mandelTest/solution_fullycoupled_10000.tex <==
\begin{tikzpicture}
  \begin{axis}[%
    width=\textwidth,
    height=\textwidth,
    xmin=0,
    xmax=1,
    xlabel style={font=\color{white!15!black}},
    xlabel={$x$},
    ymin=0,
    ymax=0.90,
    axis background/.style={fill=white},
    legend style={font=\small},
    tick label style={font=\small},
    label style={font=\small},
    ]
    \addplot [color=mycolor2, draw=none, mark=o, mark options={solid, mycolor2}]
    table[]{plotData/mandelTest/Polymesher20/solution_fullycoupled_10000-1.tsv};
    \addlegendentry{\texttt{Polymesher20}.}

    \addplot [color=mycolor3, draw=none, mark=square, mark options={solid, mycolor3}]
    table[]{plotData/mandelTest/Polymesher1/solution_fullycoupled_10000-1.tsv};
    \addlegendentry{\texttt{Polymesher1}.}

    \addplot [color=mycolor1]
    table[]{plotData/mandelTest/Polymesher20/solution_fullycoupled_10000-2.tsv};
    \addlegendentry{Exact solution.}

  \end{axis}
\end{tikzpicture}%
